Test-Time Dynamic Image Fusion

The inherent challenge of image fusion lies in capturing the correlation of multi-source images and comprehensively integrating effective information from different sources. Most existing techniques fail to perform dynamic image fusion while notably lacking theoretical guarantees, leading to potential deployment risks in this field. Is it possible to conduct dynamic image fusion with a clear theoretical justification? In this paper, we give our solution from a generalization perspective. We proceed to reveal the generalized form of image fusion and derive a new test-time dynamic image fusion paradigm. It provably reduces the upper bound of generalization error. Specifically, we decompose the fused image into multiple components corresponding to its source data. The decomposed components represent the effective information from the source data, thus the gap between them reflects the Relative Dominability (RD) of the uni-source data in constructing the fusion image. Theoretically, we prove that the key to reducing generalization error hinges on the negative correlation between the RD-based fusion weight and the uni-source reconstruction loss. Intuitively, RD dynamically highlights the dominant regions of each source and can be naturally converted to the corresponding fusion weight, achieving robust results. Extensive experiments and discussions with in-depth analysis on multiple benchmarks confirm our findings and superiority. Our code is available at https://github.com/Yinan-Xia/TTD.

==> bib.tex <==
@inproceedings{hwang2015multispectral,
  title={Multispectral pedestrian detection: Benchmark dataset and baseline},
  author={Hwang, Soonmin and Park, Jaesik and Kim, Namil and Choi, Yukyung and So Kweon, In},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1037--1045},
  year={2015}
}
@article{bulanon2009image,
  title={Image fusion of visible and thermal images for fruit detection},
  author={Bulanon, DM and Burks, TF and Alchanatis, V},
  journal={Biosystems engineering},
  volume={103},
  number={1},
  pages={12--22},
  year={2009},
  publisher={Elsevier}
}
@inproceedings{zhang2020vifb,
  title={VIFB: A visible and infrared image fusion benchmark},
  author={Zhang, Xingchen and Ye, Ping and Xiao, Gang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={104--105},
  year={2020}
}
@inproceedings{jia2021llvip,
  title={LLVIP: A visible-infrared paired dataset for low-light vision},
  author={Jia, Xinyu and Zhu, Chuang and Li, Minzhen and Tang, Wenqi and Zhou, Wenli},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={3496--3504},
  year={2021}
}
@article{10.1117/1.OE.51.1.010901,
author = {Alexander Toet and Maarten A. Hogervorst},
title = {{Progress in color night vision}},
volume = {51},
journal = {Optical Engineering},
number = {1},
publisher = {SPIE},
pages = {010901},
keywords = {image fusion, color fusion, false color, color mapping, real-time fusion, night vision, Image fusion, Visualization, RGB color model, Night vision, Sensors, Image sensors, Near infrared, Thermography, Image enhancement, Long wavelength infrared},
year = {2012},
doi = {10.1117/1.OE.51.1.010901},
URL = {https://doi.org/10.1117/1.OE.51.1.010901}
}
@inproceedings{liu2022target,
  title={Target-aware Dual Adversarial Learning and a Multi-scenario Multi-Modality Benchmark to Fuse Infrared and Visible for Object Detection},
  author={Liu, Jinyuan and Fan, Xin and Huang, Zhanbo and Wu, Guanyao and Liu, Risheng and Zhong, Wei and Luo, Zhongxuan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={5802--5811},
  year={2022}
}
@article{li2018densefuse,
  title={DenseFuse: A Fusion Approach to Infrared and Visible Images},
  author={Li, Hui and Wu, Xiao-Jun},
  journal={IEEE Transactions on Image Processing},
  volume={28},
  number={5},
  pages={2614--2623},
  month={May},
  year={2019},
  publisher={IEEE}
}
@InProceedings{Zhao_2023_CVPR,
    author    = {Zhao, Zixiang and Bai, Haowen and Zhang, Jiangshe and Zhang, Yulun and Xu, Shuang and Lin, Zudi and Timofte, Radu and Van Gool, Luc},
    title     = {CDDFuse: Correlation-Driven Dual-Branch Feature Decomposition for Multi-Modality Image Fusion},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2023},
    pages     = {5906-5916}
}
@article{xu2020u2fusion,
  title={U2Fusion: A unified unsupervised image fusion network},
  author={Xu, Han and Ma, Jiayi and Jiang, Junjun and Guo, Xiaojie and Ling, Haibin},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={44},
  number={1},
  pages={502--518},
  year={2020},
  publisher={IEEE}
}
@inproceedings{zhao2023ddfm,
  title={DDFM: denoising diffusion model for multi-modality image fusion},
  author={Zhao, Zixiang and Bai, Haowen and Zhu, Yuanzhi and Zhang, Jiangshe and Xu, Shuang and Zhang, Yulun and Zhang, Kai and Meng, Deyu and Timofte, Radu and Van Gool, Luc},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={8082--8093},
  year={2023}
}
@inproceedings{liang2022fusion,
  title={Fusion from decomposition: A self-supervised decomposition approach for image fusion},
  author={Liang, Pengwei and Jiang, Junjun and Liu, Xianming and Ma, Jiayi},
  booktitle={European Conference on Computer Vision},
  pages={719--735},
  year={2022},
  organization={Springer}
}
@article{tang2023divfusion,
  title={DIVFusion: Darkness-free infrared and visible image fusion},
  author={Tang, Linfeng and Xiang, Xinyu and Zhang, Hao and Gong, Meiqi and Ma, Jiayi},
  journal={Information Fusion},
  volume={91},
  pages={477--493},
  year={2023},
  publisher={Elsevier}
}
@inproceedings{cao2023multi,
  title={Multi-modal gated mixture of local-to-global experts for dynamic image fusion},
  author={Cao, Bing and Sun, Yiming and Zhu, Pengfei and Hu, Qinghua},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={23555--23564},
  year={2023}
}
@article{cheng2023mufusion,
  title={MUFusion: A general unsupervised image fusion network based on memory unit},
  author={Cheng, Chunyang and Xu, Tianyang and Wu, Xiao-Jun},
  journal={Information Fusion},
  volume={92},
  pages={80--92},
  year={2023},
  publisher={Elsevier}
}
@article{tang2022piafusion,
  title={PIAFusion: A progressive infrared and visible image fusion network based on illumination aware},
  author={Tang, Linfeng and Yuan, Jiteng and Zhang, Hao and Jiang, Xingyu and Ma, Jiayi},
  journal={Information Fusion},
  volume={83},
  pages={79--92},
  year={2022},
  publisher={Elsevier}
}
@article{zhang2020ifcnn,
  title={IFCNN: A general image fusion framework based on convolutional neural network},
  author={Zhang, Yu and Liu, Yu and Sun, Peng and Yan, Han and Zhao, Xiaolin and Zhang, Li},
  journal={Information Fusion},
  volume={54},
  pages={99--118},
  year={2020},
  publisher={Elsevier}
}
@article{wang2022swinfuse,
  title={SwinFuse: A residual swin transformer fusion network for infrared and visible images},
  author={Wang, Zhishe and Chen, Yanlin and Shao, Wenyu and Li, Hui and Zhang, Lei},
  journal={IEEE Transactions on Instrumentation and Measurement},
  volume={71},
  pages={1--12},
  year={2022},
  publisher={IEEE}
}
@inproceedings{zhu2024task,
  title={Task-customized mixture of adapters for general image fusion},
  author={Zhu, Pengfei and Sun, Yang and Cao, Bing and Hu, Qinghua},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7099--7108},
  year={2024}
}
@article{chen2020infrared,
  title={Infrared and visible image fusion based on target-enhanced multiscale transform decomposition},
  author={Chen, Jun and Li, Xuejiao and Luo, Linbo and Mei, Xiaoguang and Ma, Jiayi},
  journal={Information Sciences},
  volume={508},
  pages={64--78},
  year={2020},
  publisher={Elsevier}
}
@article{zhang2018sparse,
  title={Sparse representation based multi-sensor image fusion for multi-focus and multi-modality images: A review},
  author={Zhang, Qiang and Liu, Yi and Blum, Rick S and Han, Jungong and Tao, Dacheng},
  journal={Information Fusion},
  volume={40},
  pages={57--75},
  year={2018},
  publisher={Elsevier}
}
@article{zhang1999categorization,
  title={A categorization of multiscale-decomposition-based image fusion schemes with a performance study for a digital camera application},
  author={Zhang, Zhong and Blum, Rick S},
  journal={Proceedings of the IEEE},
  volume={87},
  number={8},
  pages={1315--1326},
  year={1999},
  publisher={IEEE}
}
@article{liu2017multi,
  title={Multi-focus image fusion with a deep convolutional neural network},
  author={Liu, Yu and Chen, Xun and Peng, Hu and Wang, Zengfu},
  journal={Information Fusion},
  volume={36},
  pages={191--207},
  year={2017},
  publisher={Elsevier}
}
@article{ma2019fusiongan,
  title={FusionGAN: A generative adversarial network for infrared and visible image fusion},
  author={Ma, Jiayi and Yu, Wei and Liang, Pengwei and Li, Chang and Jiang, Junjun},
  journal={Information fusion},
  volume={48},
  pages={11--26},
  year={2019},
  publisher={Elsevier}
}
@article{han2022trusted,
  title={Trusted multi-view classification with dynamic evidential fusion},
  author={Han, Zongbo and Zhang, Changqing and Fu, Huazhu and Zhou, Joey Tianyi},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={45},
  number={2},
  pages={2551--2566},
  year={2022},
  publisher={IEEE}
}
@inproceedings{han2022multimodal,
  title={Multimodal dynamics: Dynamical fusion for trustworthy multimodal classification},
  author={Han, Zongbo and Yang, Fan and Huang, Junzhou and Zhang, Changqing and Yao, Jianhua},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={20707--20717},
  year={2022}
}
@inproceedings{xue2023dynamic,
  title={Dynamic multimodal fusion},
  author={Xue, Zihui and Marculescu, Radu},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2574--2583},
  year={2023}
}
@inproceedings{gao2019dynamic,
  title={Dynamic fusion with intra-and inter-modality attention flow for visual question answering},
  author={Gao, Peng and Jiang, Zhengkai and You, Haoxuan and Lu, Pan and Hoi, Steven CH and Wang, Xiaogang and Li, Hongsheng},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={6639--6648},
  year={2019}
}
@inproceedings{yu2023adaptive,
  title={Adaptive Fusion for Visual Question Answering: Integrating Multi-Label Classification and Similarity Matching},
  author={Yu, Zhengtao and Zhao, Jia and Wang, Huiling and Guo, Chenliang and Zhou, Tong and Sun, Chongxiang},
  booktitle={Proceedings of the 5th ACM International Conference on Multimedia in Asia},
  pages={1--7},
  year={2023}
}

@article{Zhang_2021,   
title={Benchmarking and Comparing Multi-exposure Image Fusion Algorithms},  
url={http://dx.doi.org/10.1016/j.inffus.2021.02.005},  
DOI={10.1016/j.inffus.2021.02.005},
journal={Information Fusion},
author={Zhang, Xingchen},
year={2021},  month={Oct},
pages={111–131},
language={en-US}
}
 @article{Zhang_Le_Shao_Xu_Ma_2021,  
 title={MFF-GAN: An unsupervised generative adversarial network with adaptive and gradient joint constraints for multi-focus image fusion}, 
 url={http://dx.doi.org/10.1016/j.inffus.2020.08.022}, 
 DOI={10.1016/j.inffus.2020.08.022}, 
 journal={Information Fusion}, 
 author={Zhang, Hao and Le, Zhuliang and Shao, Zhenfeng and Xu, Han and Ma, Jiayi}, 
 year={2021}, 
 month={Feb}, 
 pages={40–53}, 
 language={en-US} 
 }
@article{collins2000system,
  title={A system for video surveillance and monitoring},
  author={Collins, Robert T and Lipton, Alan J and Kanade, Takeo and Fujiyoshi, Hironobu and Duggins, David and Tsin, Yanghai and Tolliver, David and Enomoto, Nobuyoshi and Hasegawa, Osamu and Burt, Peter and others},
  journal={VSAM final report},
  volume={2000},
  number={1-68},
  pages={1},
  year={2000},
  publisher={Citeseer}
}
@inproceedings{li2009towards,
  title={Towards total scene understanding: Classification, annotation and segmentation in an automatic framework},
  author={Li, Li-Jia and Socher, Richard and Fei-Fei, Li},
  booktitle={2009 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2036--2043},
  year={2009},
  organization={IEEE}
}
@article{james2014medical,
  title={Medical image fusion: A survey of the state of the art},
  author={James, Alex Pappachen and Dasarathy, Belur V},
  journal={Information fusion},
  volume={19},
  pages={4--19},
  year={2014},
  publisher={Elsevier}
}
@article{ma2019infrared,
  title={Infrared and visible image fusion methods and applications: A survey},
  author={Ma, Jiayi and Ma, Yong and Li, Chang},
  journal={Information fusion},
  volume={45},
  pages={153--178},
  year={2019},
  publisher={Elsevier}
}
@article{Ma2015MultiExposure,
  author={Ma, Kede and Zeng, Kai and Wang, Zhou},
  journal={IEEE Transactions on Image Processing}, 
  title={Perceptual Quality Assessment for Multi-Exposure Image Fusion}, 
  year={2015},
  volume={24},
  number={11},
  pages={3345-3356},
  keywords={Image fusion;Databases;Quality assessment;Computational modeling;Image sequences;Prediction algorithms;Image edge detection;Multi-exposure image fusion (MEF);image quality assessment;structural similarity;luminance consistency;subjective evaluations,;perceptual image processing;Multi-exposure image fusion (MEF);image quality assessment;structural similarity;luminance consistency;subjective evaluations;perceptual image processing},
  doi={10.1109/TIP.2015.2442920}}
@book{mohri2018foundations,
  title={Foundations of machine learning},
  author={Mohri, Mehryar and Rostamizadeh, Afshin and Talwalkar, Ameet},
  year={2018},
  publisher={MIT press}
}
@article{zhao2020didfuse,
  title={DIDFuse: Deep image decomposition for infrared and visible image fusion},
  author={Zhao, Zixiang and Xu, Shuang and Zhang, Chunxia and Liu, Junmin and Li, Pengfei and Zhang, Jiangshe},
  journal={arXiv preprint arXiv:2003.09210},
  year={2020}
}
@inproceedings{zhang2020rethinking,
  title={Rethinking the image fusion: A fast unified image fusion network based on proportional maintenance of gradient and intensity},
  author={Zhang, Hao and Xu, Han and Xiao, Yang and Guo, Xiaojie and Ma, Jiayi},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={34},
  pages={12797--12804},
  year={2020}
}
@article{lu2021learning,
  title={Learning nonlinear operators via DeepONet based on the universal approximation theorem of operators},
  author={Lu, Lu and Jin, Pengzhan and Pang, Guofei and Zhang, Zhongqiang and Karniadakis, George Em},
  journal={Nature machine intelligence},
  volume={3},
  number={3},
  pages={218--229},
  year={2021},
  publisher={Nature Publishing Group UK London}
}

@article{eskicioglu1995image,
  title={Image quality measures and their performance},
  author={Eskicioglu, Ahmet M and Fisher, Paul S},
  journal={IEEE Transactions on communications},
  volume={43},
  number={12},
  pages={2959--2965},
  year={1995},
  publisher={IEEE}
}

@article{Cui_Feng_Xu_Li_Chen_2015,  
 title={Detail preserved fusion of visible and infrared images using regional saliency extraction and multi-scale image decomposition}, 
 url={http://dx.doi.org/10.1016/j.optcom.2014.12.032}, 
 DOI={10.1016/j.optcom.2014.12.032}, 
 journal={Optics Communications}, 
 author={Cui, Guangmang and Feng, Huajun and Xu, Zhihai and Li, Qi and Chen, Yueting}, 
 year={2015}, 
 month={Apr}, 
 pages={199–209}, 
 language={en-US} 
 }
@article{Aslantas_Bendes_2015,  
 title={A new image quality metric for image fusion: The sum of the correlations of differences}, 
 url={http://dx.doi.org/10.1016/j.aeue.2015.09.004}, 
 DOI={10.1016/j.aeue.2015.09.004}, 
 journal={AEU - International Journal of Electronics and Communications}, 
 author={Aslantas, V. and Bendes, E.}, 
 year={2015}, 
 month={Dec}, 
 pages={1890–1896}, 
 language={en-US} 
 }
 @article{Wang_Bovik_Sheikh_Simoncelli_2004,  
 title={Image Quality Assessment: From Error Visibility to Structural Similarity}, 
 url={http://dx.doi.org/10.1109/tip.2003.819861}, 
 DOI={10.1109/tip.2003.819861}, 
 journal={IEEE Transactions on Image Processing}, 
 author={Wang, Z. and Bovik, A.C. and Sheikh, H.R. and Simoncelli, E.P.}, 
 year={2004}, 
 month={Apr}, 
 pages={600–612}, 
 language={en-US} 
 }
@article{roberts2008assessment,
  title={Assessment of image fusion procedures using entropy, image quality, and multispectral classification},
  author={Roberts, J Wesley and Van Aardt, Jan A and Ahmed, Fethi Babikker},
  journal={Journal of Applied Remote Sensing},
  volume={2},
  number={1},
  pages={023522},
  year={2008},
  publisher={SPIE}
}
@inproceedings{zhang2017convexified,
  title={Convexified convolutional neural networks},
  author={Zhang, Yuchen and Liang, Percy and Wainwright, Martin J},
  booktitle={International Conference on Machine Learning},
  pages={4044--4053},
  year={2017},
  organization={PMLR}
}
@inproceedings{zhang2023provable,
  title={Provable dynamic fusion for low-quality multimodal data},
  author={Zhang, Qingyang and Wu, Haitao and Zhang, Changqing and Hu, Qinghua and Fu, Huazhu and Zhou, Joey Tianyi and Peng, Xi},
  booktitle={International conference on machine learning},
  pages={41753--41769},
  year={2023},
  organization={PMLR}
}
@inproceedings{gokberk2006comparative,
  title={Comparative analysis of decision-level fusion algorithms for 3D face recognition},
  author={Gokberk, Berk and Akarun, Lale},
  booktitle={18th International Conference on Pattern Recognition (ICPR'06)},
  volume={3},
  pages={1018--1021},
  year={2006},
  organization={IEEE}
}
@book{nixon2019feature,
  title={Feature extraction and image processing for computer vision},
  author={Nixon, Mark and Aguado, Alberto},
  year={2019},
  publisher={Academic press}
}
@article{niyogi1996relationship,
  title={On the relationship between generalization error, hypothesis complexity, and sample complexity for radial basis functions},
  author={Niyogi, Partha and Girosi, Federico},
  journal={Neural Computation},
  volume={8},
  number={4},
  pages={819--842},
  year={1996},
  publisher={MIT Press}
}
@article{xu2022multi,
  title={Multi-exposure image fusion techniques: A comprehensive review},
  author={Xu, Fang and Liu, Jinghong and Song, Yueming and Sun, Hui and Wang, Xuan},
  journal={Remote Sensing},
  volume={14},
  number={3},
  pages={771},
  year={2022},
  publisher={MDPI}
}
@inproceedings{ram2017deepfuse,
  title={Deepfuse: A deep unsupervised approach for exposure fusion with extreme exposure image pairs},
  author={Ram Prabhakar, K and Sai Srikar, V and Venkatesh Babu, R},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={4714--4722},
  year={2017}
}
@article{wang2019detail,
  title={Detail-enhanced multi-scale exposure fusion in YUV color space},
  author={Wang, Qiantong and Chen, Weihai and Wu, Xingming and Li, Zhengguo},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  volume={30},
  number={8},
  pages={2418--2429},
  year={2019},
  publisher={IEEE}
}
@article{liu2015dense,
  title={Dense SIFT for ghost-free multi-exposure fusion},
  author={Liu, Yu and Wang, Zengfu},
  journal={Journal of Visual Communication and Image Representation},
  volume={31},
  pages={208--224},
  year={2015},
  publisher={Elsevier}
}
@inproceedings{lee2018multi,
  title={A multi-exposure image fusion based on the adaptive weights reflecting the relative pixel intensity and global gradient},
  author={Lee, Sang-hoon and Park, Jae Sung and Cho, Nam Ik},
  booktitle={2018 25th IEEE international conference on image processing (ICIP)},
  pages={1737--1741},
  year={2018},
  organization={IEEE}
}
@inproceedings{li2018multi,
  title={Multi-exposure fusion with CNN features},
  author={Li, Hui and Zhang, Lei},
  booktitle={2018 25th IEEE International Conference on Image Processing (ICIP)},
  pages={1723--1727},
  year={2018},
  organization={IEEE}
}
@article{ma2017multi,
  title={Multi-exposure image fusion by optimizing a structural similarity index},
  author={Ma, Kede and Duanmu, Zhengfang and Yeganeh, Hojatollah and Wang, Zhou},
  journal={IEEE Transactions on Computational Imaging},
  volume={4},
  number={1},
  pages={60--72},
  year={2017},
  publisher={IEEE}
}
@article{lei2023galfusion,
  title={GALFusion: Multi-exposure image fusion via a global--local aggregation learning network},
  author={Lei, Jia and Li, Jiawei and Liu, Jinyuan and Zhou, Shihua and Zhang, Qiang and Kasabov, Nikola K},
  journal={IEEE Transactions on Instrumentation and Measurement},
  volume={72},
  pages={1--15},
  year={2023},
  publisher={IEEE}
}
@article{liu2023holoco,
  title={HoLoCo: Holistic and local contrastive learning network for multi-exposure image fusion},
  author={Liu, Jinyuan and Wu, Guanyao and Luan, Junsheng and Jiang, Zhiying and Liu, Risheng and Fan, Xin},
  journal={Information Fusion},
  volume={95},
  pages={237--249},
  year={2023},
  publisher={Elsevier}
}
@article{li2020drpl,
  title={DRPL: Deep regression pair learning for multi-focus image fusion},
  author={Li, Jinxing and Guo, Xiaobao and Lu, Guangming and Zhang, Bob and Xu, Yong and Wu, Feng and Zhang, David},
  journal={IEEE Transactions on Image Processing},
  volume={29},
  pages={4816--4831},
  year={2020},
  publisher={IEEE}
}
@article{amin2019ensemble,
  title={Ensemble of CNN for multi-focus image fusion},
  author={Amin-Naji, Mostafa and Aghagolzadeh, Ali and Ezoji, Mehdi},
  journal={Information fusion},
  volume={51},
  pages={201--214},
  year={2019},
  publisher={Elsevier}
}
@article{xu2020deep,
  title={A deep model for multi-focus image fusion based on gradients and connected regions},
  author={Xu, Han and Fan, Fan and Zhang, Hao and Le, Zhuliang and Huang, Jun},
  journal={IEEE Access},
  volume={8},
  pages={26316--26327},
  year={2020},
  publisher={IEEE}
}
@article{qiu2019guided,
  title={Guided filter-based multi-focus image fusion through focus region detection},
  author={Qiu, Xiaohua and Li, Min and Zhang, Liqiong and Yuan, Xianjie},
  journal={Signal Processing: Image Communication},
  volume={72},
  pages={35--46},
  year={2019},
  publisher={Elsevier}
}
@article{lai2019multi,
  title={Multi-scale visual attention deep convolutional neural network for multi-focus image fusion},
  author={Lai, Rui and Li, Yongxue and Guan, Juntao and Xiong, Ai},
  journal={IEEE Access},
  volume={7},
  pages={114385--114399},
  year={2019},
  publisher={IEEE}
}
@inproceedings{song2019multi,
  title={Multi-focus image fusion with PCA filters of PCANet},
  author={Song, Xu and Wu, Xiao-Jun},
  booktitle={Multimodal Pattern Recognition of Social Signals in Human-Computer-Interaction: 5th IAPR TC 9 Workshop, MPRSS 2018, Beijing, China, August 20, 2018, Revised Selected Papers 5},
  pages={1--17},
  year={2019},
  organization={Springer}
}
@article{ma2021sesf,
  title={Sesf-fuse: An unsupervised deep model for multi-focus image fusion},
  author={Ma, Boyuan and Zhu, Yu and Yin, Xiang and Ban, Xiaojuan and Huang, Haiyou and Mukeshimana, Michele},
  journal={Neural Computing and Applications},
  volume={33},
  pages={5793--5804},
  year={2021},
  publisher={Springer}
}
@article{ma2019multi,
  title={Multi-focus image fusion using boosted random walks-based algorithm with two-scale focus maps},
  author={Ma, Jinlei and Zhou, Zhiqiang and Wang, Bo and Miao, Lingjuan and Zong, Hua},
  journal={Neurocomputing},
  volume={335},
  pages={9--20},
  year={2019},
  publisher={Elsevier}
}
@article{liu2021learning,
  title={Learning a deep multi-scale feature ensemble and an edge-attention guidance for image fusion},
  author={Liu, Jinyuan and Fan, Xin and Jiang, Ji and Liu, Risheng and Luo, Zhongxuan},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  volume={32},
  number={1},
  pages={105--119},
  year={2021},
  publisher={IEEE}
}
@article{liu2022attention,
  title={Attention-guided global-local adversarial learning for detail-preserving multi-exposure image fusion},
  author={Liu, Jinyuan and Shang, Jingjie and Liu, Risheng and Fan, Xin},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  volume={32},
  number={8},
  pages={5026--5040},
  year={2022},
  publisher={IEEE}
}
@article{du2016overview,
  title={An overview of multi-modal medical image fusion},
  author={Du, Jiao and Li, Weisheng and Lu, Ke and Xiao, Bin},
  journal={Neurocomputing},
  volume={215},
  pages={3--20},
  year={2016},
  publisher={Elsevier}
}
@inproceedings{cao2020generalization,
  title={Generalization error bounds of gradient descent for learning over-parameterized deep relu networks},
  author={Cao, Yuan and Gu, Quanquan},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  pages={3349--3356},
  year={2020}
}
@inproceedings{lugosi2022generalization,
  title={Generalization bounds via convex analysis},
  author={Lugosi, G{\'a}bor and Neu, Gergely},
  booktitle={Conference on Learning Theory},
  pages={3524--3546},
  year={2022},
  organization={PMLR}
}
